Unsupervised Contrastive Domain Adaptation for Semantic Segmentation

Semantic segmentation models struggle to generalize in the presence of domain shift. In this paper, we introduce contrastive learning for feature alignment in cross-domain adaptation. We assemble both in-domain contrastive pairs and cross-domain contrastive pairs to learn discriminative features that align across domains. Based on the resulting well-aligned feature representations we introduce a label expansion approach that is able to discover samples from hard classes during the adaptation process to further boost performance. The proposed approach consistently outperforms state-of-the-art methods for domain adaptation. It achieves 60.2% mIoU on the Cityscapes dataset when training on the synthetic GTA5 dataset together with unlabeled Cityscapes images.

==> tex/fig_dist.tex <==
\begin{figure*}[t]
\centering

 \includegraphics[width=0.32\linewidth]{DoCo/images/dist/dist_org2.png}
 \includegraphics[width=0.32\linewidth]{DoCo/images/dist/dist_sota2.png}
 \includegraphics[width=0.32\linewidth]{DoCo/images/dist/dist_ours2.png}\\
  \includegraphics[width=0.8\linewidth]{DoCo/images/dist/color_tag.png}

	\caption{\small  Distance between the class prototypes of different domains (Cityscapes and GTA5). We compute the class prototypes for 19 categories in the GTA5 dataset and another 19 category centers for the real Cityscapes dataset. We then measure $L_2$ distances between the class prototypes  (GTA5 to Cityscapes). The prototype of each class in different domains are making much closer by our domain contrastive strategy.}
	\label{fig:feature_distance}
\end{figure*}
